How Close is a Tree to a Euclidean Minimum Spanning Tree?

Let $\Gamma$ be a straight-line crossing-free drawing of a tree $T$. A \emph{bad pair} in $\Gamma$ is a pair of non-adjacent vertices of $T$ whose Euclidean distance in $\Gamma$ is smaller than the length of the longest edge in the path connecting them in~$\Gamma$. When $\Gamma$ has no bad pairs, $\Gamma$ is a Euclidean Minimum Spanning Tree of its vertex set (or EMST-drawing for short). Deciding whether a tree of maximum degree at most six admits an EMST-drawing is known to be \NP-hard. In contrast, we characterize those caterpillars that admit an EMST-drawing. The characterization gives rise to a linear-time algorithm that decides if a caterpillar admits an EMST-drawing, and in the affirmative case, computes such a drawing. For caterpillars of maximum degree six, we further present a linear-time algorithm to compute a crossing-free straight-line drawing with the minimum number of bad pairs. For $n$-vertex trees with maximum vertex degree $\Delta$, we prove the $\Delta^2n\log n$ upper bound on the minimum number of bad pairs. In the special case of stars, we construct a drawing with the minimum number of bad pairs.

==> macros.tex <==
\usepackage{a4wide}

\usepackage{amssymb,amsthm,amsmath}
\usepackage{thmtools}
\usepackage{xcolor,xspace}
\usepackage[linesnumbered, lined, boxed]{algorithm2e}
\usepackage[colorlinks=true, urlcolor=Blue, citecolor=blue, linkcolor=blue, pdfencoding=auto, psdextra]{hyperref}
\usepackage[capitalize,nameinlink]{cleveref}
\usepackage{graphicx}
\usepackage{todonotes}
%\usepackage{ulem}
\usepackage{comment}
\usepackage{caption, subcaption}
\usepackage{complexity}
\usepackage{boxedminipage}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{rr}{Reduction Rule}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}


\theoremstyle{remark}
\newtheorem{claim}{Claim}
\newtheorem{claimproof}{Proof of claim}
%
% the following line ensures that the proof of the claim uses the number from the directly preceding claim
%
\renewcommand{\theclaimproof}{\theclaim}
\Crefname{claim}{Claim}{Claims}

\usepackage{etoolbox}
\AtEndEnvironment{proof}{\setcounter{claim}{0} \setcounter{claimproof}{0}}
\AtEndEnvironment{claimproof}{\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill\quad\hbox{$\blacksquare$}}

%\newenvironment{claim}[1]{\par\noindent\underline{Claim:}\space#1}{}
%\newenvironment{claimproof}[1]{\par\noindent\underline{Proof:}\space#1}{\hfill $\blacksquare$}

\newcommand{\resolved}[1]{\todo[color=green!40]{#1}}
\newcommand{\bpn}{\operatorname{bp}}

\newcommand{\yes}{\textsf{YES}}
\newcommand{\no}{\textsf{NO}}
\newcommand{\fpt}{\textsf{FPT}\xspace}

\newcommand{\floor}[1]{{\left\lfloor #1 \right\rfloor}}
\newcommand{\set}[1]{{\left\{ #1 \right\}}}
\newcommand{\Oh}[1]{O\left(#1\right)}

\newcommand{\problem}[3]{
        \begin{center}
                \begin{boxedminipage}{0.99\textwidth}
                        \textsc{#1}
                        
                        \vspace{2pt}
                        
                        \begin{tabular}{l p{0.8\textwidth}}
                                \textit{Instance:} & {#2}\\
                                
                                \textit{Question:} & {#3}
                        \end{tabular}
                \end{boxedminipage}
        \end{center}
}



